Power of Ensemble Diversity and Randomization for Energy Aggregation

We study an ensemble of diverse (inhomogeneous) thermostatically controlled loads aggregated to provide the demand response (DR) services in a district-level energy system. Each load in the ensemble is assumed to be equipped with a random number generator switching heating/cooling on or off with a Poisson rate, $r$, when the load leaves the comfort zone. Ensemble diversity is modeled through inhomogeneity/disorder in the deterministic dynamics of loads. Approached from the standpoint of statistical physics, the ensemble represents a non-equilibrium system driven away from its natural steady state by the DR. The ability of the ensemble to recover by mixing faster to the steady state after its DR's use is advantageous. The trade-off between the level of the aggregator's control, commanding the devices to lower the rate $r$, and the phase-space-oscillatory deterministic dynamics is analyzed. We discover that there exists a critical value, $r_c$, corresponding to both the most efficient mixing and the bifurcation point where the ensemble transitions from the oscillatory relaxation at $r>r_c$ to the pure relaxation at $r<r_c$. Then, we study the effect of the load diversity, investigating four different disorder probability distributions (DPDs) ranging from the case of the Gaussian DPD to the case of the uniform with finite support DPD. Demonstrating resemblance to the similar question of the effectiveness of Landau damping in plasma physics, we show that stronger regularity of the DPD around its maximum results in faster mixing. Our theoretical analysis is supported by extensive numerical validation, which also allows us to access the effect of the ensemble's finite size.

==> preambule.tex <==

\RequirePackage[T1]{fontenc}
\RequirePackage[utf8]{inputenc}
\RequirePackage[english]{babel} 
%\RequirePackage[english,francais]{babel} 
%\usepackage[utf8]{inputenc}      % utilisation directe des caractères accentués sur pc
\usepackage{graphics,graphicx,epsfig,subfigure}
\usepackage{times}
\usepackage{bookmark}%Used for the ToC

%\usepackage{tocbibind}%add ToC in Toc
%\usepackage{cleveref}
\RequirePackage{fancyhdr}			% gestion de l'en-tête et du pied de page
\RequirePackage{geometry}			% gestion des marges et autres (permet de définir le format du document)

\RequirePackage{engrec}				% pour utiliser des compteurs avec des lettres grecques
\RequirePackage{fmtcount}		    % pour utiliser des compteurs en toute lettre (Un,Deux,...)

%\RequirePackage[backref]{hyperref}
%\usepackage[newparttoc]{titlesec}% http://ctan.org/pkg/titlesec

\RequirePackage{apptools}	% Pour utiliser la commande AtAppendix 	
%\makeatletter
%\usepackage{caption}
%\usepackage{subcaption}

% quelques package utiles

\usepackage{graphicx} % inclusion des figures
\usepackage{amsthm}    %Pour théorème et tout
\usepackage{amsmath} % collection de symboles mathématiques
\usepackage{amssymb} % collection de symboles mathématiques
\usepackage{array}
\usepackage{tabularx}

%\usepackage{indentfirst}
\usepackage{booktabs}
\usepackage{ulem}%barré du texte
\usepackage{bbm}

\usepackage{bibunits} %bibliographie par partie
%\usepackage{subfigure}
%\usepackage{psfrag} % remplacement du texte d'une figure ps par du texte latex
\usepackage{sistyle} % mise en forme des unités

\usepackage{eurosym} % symbole 
\def\{\euro{}}
%\usepackage{picins}

\usepackage{color} % gestion de différentes couleurs

\usepackage{mathrsfs} %jolie lettres



%%% I use this part to make annotation in color to myself. With the balise \dm{blabla} (in green) or \dmref{}  \dmb{}
\definecolor{David}{rgb}{0,.8,.5}
\newcommand{\dm}[1]{{\color{green} #1}}
\definecolor{Julien}{rgb}{1,.4,.3}
\newcommand{\dmref}[1]{{\color{red} #1}}
\newcommand{\dmb}[1]{{\color{blue} #1}}


%I use the following command to force the break after the balise Remark (but it does not always works)
\newtheoremstyle{break}
  {\topsep}{\topsep}%
  {}{}%
  {\bfseries}{}%
  {\newline}{}%
  
\theoremstyle{break}
%I create my theorem, remark, ... environment (can be modified)
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{remark}{Remark}[chapter]
%\newtheorem{theorem*}{Theorem*}
%\newtheorem{remark*}[theorem]{Remark}
%\newtheorem{conjecture}{Conjecture}[chapter]

\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}} %Use to create nice table 


\newenvironment{sciabstract}{%
\begin{quote} \bf}
{\end{quote}}

%%Here I put all my prefered shortcuts

\newcommand{\eg}{e.g.~}
\newcommand{\ie}{i.e.~}
\renewcommand{\d}{\mathrm{d}} %straight d for integrals and derivatites please! (\d t, \d x, ...)
\renewcommand{\Re}{\operatorname{Re}} %partie réelle d'un complexe
\renewcommand{\Im}{\operatorname{Im}} %partie imaginaire d'un complexe
\newcommand{\res}{\operatorname{Res}}
\newcommand{\PV}{\operatorname{PV}}
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\erfc}{\operatorname{erfc}}


\newcommand{\w}{\mathrm{w}}
\newcommand{\W}{\mathrm{W}}
\renewcommand{\P}{\mathscr{P}}
\renewcommand{\L}{\operatorname{\mathscr{L}}}
\newcommand{\N}{\operatorname{\mathscr{N}}}
\renewcommand\O[1]{\mathrm{O}\left (#1\right )}
\renewcommand\o[1]{\mathrm{o}\left (#1\right )}
% \renewcommand{\r}{\vec{r}}
% \renewcommand{\v}{\vec{v}}
% \renewcommand{\k}{\vec{k}}

\newcommand{\kb}{k_{\text{B}}}
\newcommand{\F}{\mathrm{F}}
\newcommand{\Fc}{\vec{\F}_{\rm{c}}}
\newcommand{\Fs}{\vec{\F}_{\rm{s}}}
\newcommand{\phic}{\phi_{\rm{c}}}
\newcommand{\rhok}{\rho}
\newcommand{\fp}{(f^0)'}
\newcommand{\E}{\mathcal{E}}
\newcommand{\kk}{\kappa}
\newcommand{\sn}{\mathrm{sn}}
\newcommand{\cn}{\mathrm{cn}}
\newcommand{\dn}{\mathrm{dn}}
\newcommand{\fv}{f^0}
\newcommand{\fj}{F^0}
\newcommand{\fpj}{\partial_J F^0}
\newcommand{\fe}{\mathcal{F}^0}
\newcommand{\fk}{\bar{f}^0}
\newcommand{\Pc}{\Psi_c}
\newcommand{\Pct}{\tilde{\Psi}_c}
\newcommand{\psit}{\tilde{\psi}}
\newcommand{\Psit}{\widetilde{\Psi}}
\newcommand{\xit}{\tilde{\xi}}
\newcommand{\Xit}{\widetilde{\Xi}}
\newcommand{\cc}{\mathrm{c.c.}}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\cs}{\mathbbm{c}}
\newcommand{\s}{\mathbbm{s}}
\newcommand{\muc}{{\mu_c}}
\newcommand{\Pl}{\Psi^{(1)}_\muc}
\newcommand{\Po}{\Psi^{(0)}_\muc}
\newcommand{\Plt}{\widetilde{\Psi}^{(1)}_\muc}
\newcommand{\Pot}{\widetilde{\Psi}^{(0)}_\muc}
\newcommand{\dL}{\Delta\!\L}
\newcommand{\B}{\mathscr{B}}

\newcommand{\xid}{\xi_{\downarrow}}
\newcommand{\xiu}{\xi_{\uparrow}}
\newcommand{\xd}{x_{\downarrow}}
\newcommand{\xu}{x_{\uparrow}}
